Two Sample Inference for Populations of Graphical Models with Applications to Functional Connectivity

Gaussian Graphical Models (GGM) are popularly used in neuroimaging studies based on fMRI, EEG or MEG to estimate functional connectivity, or relationships between remote brain regions. In multi-subject studies, scientists seek to identify the functional brain connections that are different between two groups of subjects, i.e. connections present in a diseased group but absent in controls or vice versa. This amounts to conducting two-sample large scale inference over network edges post graphical model selection, a novel problem we call Population Post Selection Inference. Current approaches to this problem include estimating a network for each subject, and then assuming the subject networks are fixed, conducting two-sample inference for each edge. These approaches, however, fail to account for the variability associated with estimating each subject's graph, thus resulting in high numbers of false positives and low statistical power. By using resampling and random penalization to estimate the post selection variability together with proper random effects test statistics, we develop a new procedure we call $R^{3}$ that solves these problems. Through simulation studies we show that $R^{3}$ offers major improvements over current approaches in terms of error control and statistical power. We apply our method to identify functional connections present or absent in autistic subjects using the ABIDE multi-subject fMRI study.

==> abstract.tex <==
\begin{abstract}
~Gaussian Graphical Models (GGM) are popularly used in neuroimaging
studies based on fMRI, EEG or MEG to estimate functional connectivity,
or relationships between remote brain regions. In multi-subject
studies, scientists seek to identify the functional brain connections
that are different between two groups of subjects, i.e. connections
present in a diseased group but absent in controls or vice versa. This
amounts to conducting two-sample large scale inference over network
edges post graphical model selection, a novel problem we call
Population Post Selection Inference.  Current approaches to this
problem include estimating a network for each subject, and then
assuming the subject networks are fixed, conducting two-sample
inference for each edge. These approaches, however, fail to account
for the variability associated with estimating each subject's graph,
thus resulting in high numbers of false positives and low statistical
power.  By using resampling and random penalization to estimate the
post selection variability together with proper random effects test
statistics, we develop a new procedure we call $R^{3}$ that solves
these problems.  Through simulation studies we show that $R^{3}$
offers major improvements over current approaches in terms of error
control and statistical power.  We apply our
method to identify functional connections present or absent in
autistic subjects using the ABIDE multi-subject fMRI study. 
\end{abstract}

